Measurement of Groomed Jet Substructure Observables in \pp Collisions at $\sqrt{s} = 200$ GeV with STAR

In this letter, measurements of the shared momentum fraction ($z_{\rm{g}}$) and the groomed jet radius ($R_{\rm{g}}$), as defined in the SoftDrop algorihm, are reported in \pp collisions at $\sqrt{s} = 200$ GeV collected by the STAR experiment. These substructure observables are differentially measured for jets of varying resolution parameters from $R = 0.2 - 0.6$ in the transverse momentum range $15 < p_{\rm{T, jet}} < 60$ GeV$/c$. These studies show that, in the $p_{\rm{T, jet}}$ range accessible at $\sqrt{s} = 200$ GeV and with increasing jet resolution parameter and jet transverse momentum, the $z_{\rm{g}}$ distribution asymptotically converges to the DGLAP splitting kernel for a quark radiating a gluon. The groomed jet radius measurements reflect a momentum-dependent narrowing of the jet structure for jets of a given resolution parameter, i.e., the larger the $p_{\rm{T, jet}}$, the narrower the first splitting. For the first time, these fully corrected measurements are compared to Monte Carlo generators with leading order QCD matrix elements and leading log in the parton shower, and to state-of-the-art theoretical calculations at next-to-leading-log accuracy. We observe that PYTHIA 6 with parameters tuned to reproduce RHIC measurements is able to quantitatively describe data, whereas PYTHIA 8 and HERWIG 7, tuned to reproduce LHC data, are unable to provide a simultaneous description of both $z_{\rm{g}}$ and $R_{\rm{g}}$, resulting in opportunities for fine parameter tuning of these models for \pp collisions at RHIC energies. We also find that the theoretical calculations without non-perturbative corrections are able to qualitatively describe the trend in data for jets of large resolution parameters at high $p_{\rm{T, jet}}$, but fail at small jet resolution parameters and low jet transverse momenta.

==> star_authorlist_4March2020.tex <==
\author{
J.~Adam$^{6}$,
L.~Adamczyk$^{2}$,
J.~R.~Adams$^{39}$,
J.~K.~Adkins$^{30}$,
G.~Agakishiev$^{28}$,
M.~M.~Aggarwal$^{40}$,
Z.~Ahammed$^{59}$,
I.~Alekseev$^{3,35}$,
D.~M.~Anderson$^{53}$,
A.~Aparin$^{28}$,
E.~C.~Aschenauer$^{6}$,
M.~U.~Ashraf$^{11}$,
F.~G.~Atetalla$^{29}$,
A.~Attri$^{40}$,
G.~S.~Averichev$^{28}$,
V.~Bairathi$^{22}$,
K.~Barish$^{10}$,
A.~Behera$^{51}$,
R.~Bellwied$^{20}$,
A.~Bhasin$^{27}$,
J.~Bielcik$^{14}$,
J.~Bielcikova$^{38}$,
L.~C.~Bland$^{6}$,
I.~G.~Bordyuzhin$^{3}$,
J.~D.~Brandenburg$^{48,6}$,
A.~V.~Brandin$^{35}$,
J.~Butterworth$^{44}$,
H.~Caines$^{62}$,
M.~Calder{\'o}n~de~la~Barca~S{\'a}nchez$^{8}$,
D.~Cebra$^{8}$,
I.~Chakaberia$^{29,6}$,
P.~Chaloupka$^{14}$,
B.~K.~Chan$^{9}$,
F-H.~Chang$^{37}$,
Z.~Chang$^{6}$,
N.~Chankova-Bunzarova$^{28}$,
A.~Chatterjee$^{11}$,
D.~Chen$^{10}$,
J.~H.~Chen$^{18}$,
X.~Chen$^{47}$,
Z.~Chen$^{48}$,
J.~Cheng$^{55}$,
M.~Cherney$^{13}$,
M.~Chevalier$^{10}$,
S.~Choudhury$^{18}$,
W.~Christie$^{6}$,
H.~J.~Crawford$^{7}$,
M.~Csan\'{a}d$^{16}$,
M.~Daugherity$^{1}$,
T.~G.~Dedovich$^{28}$,
I.~M.~Deppner$^{19}$,
A.~A.~Derevschikov$^{42}$,
L.~Didenko$^{6}$,
X.~Dong$^{31}$,
J.~L.~Drachenberg$^{1}$,
J.~C.~Dunlop$^{6}$,
T.~Edmonds$^{43}$,
N.~Elsey$^{61}$,
J.~Engelage$^{7}$,
G.~Eppley$^{44}$,
R.~Esha$^{51}$,
S.~Esumi$^{56}$,
O.~Evdokimov$^{12}$,
A.~Ewigleben$^{32}$,
O.~Eyser$^{6}$,
R.~Fatemi$^{30}$,
S.~Fazio$^{6}$,
P.~Federic$^{38}$,
J.~Fedorisin$^{28}$,
C.~J.~Feng$^{37}$,
Y.~Feng$^{43}$,
P.~Filip$^{28}$,
E.~Finch$^{50}$,
Y.~Fisyak$^{6}$,
A.~Francisco$^{62}$,
L.~Fulek$^{2}$,
C.~A.~Gagliardi$^{53}$,
T.~Galatyuk$^{15}$,
F.~Geurts$^{44}$,
A.~Gibson$^{58}$,
K.~Gopal$^{23}$,
D.~Grosnick$^{58}$,
W.~Guryn$^{6}$,
A.~I.~Hamad$^{29}$,
A.~Hamed$^{5}$,
J.~W.~Harris$^{62}$,
S.~He$^{11}$,
W.~He$^{18}$,
X.~He$^{26}$,
S.~Heppelmann$^{8}$,
S.~Heppelmann$^{41}$,
N.~Herrmann$^{19}$,
E.~Hoffman$^{20}$,
L.~Holub$^{14}$,
Y.~Hong$^{31}$,
S.~Horvat$^{62}$,
Y.~Hu$^{18}$,
H.~Z.~Huang$^{9}$,
S.~L.~Huang$^{51}$,
T.~Huang$^{37}$,
X.~ Huang$^{55}$,
T.~J.~Humanic$^{39}$,
P.~Huo$^{51}$,
G.~Igo$^{9}$,
D.~Isenhower$^{1}$,
W.~W.~Jacobs$^{25}$,
C.~Jena$^{23}$,
A.~Jentsch$^{6}$,
Y.~JI$^{47}$,
J.~Jia$^{6,51}$,
K.~Jiang$^{47}$,
S.~Jowzaee$^{61}$,
X.~Ju$^{47}$,
E.~G.~Judd$^{7}$,
S.~Kabana$^{29}$,
M.~L.~Kabir$^{10}$,
S.~Kagamaster$^{32}$,
D.~Kalinkin$^{25}$,
K.~Kang$^{55}$,
D.~Kapukchyan$^{10}$,
K.~Kauder$^{6}$,
H.~W.~Ke$^{6}$,
D.~Keane$^{29}$,
A.~Kechechyan$^{28}$,
M.~Kelsey$^{31}$,
Y.~V.~Khyzhniak$^{35}$,
D.~P.~Kiko\l{}a~$^{60}$,
C.~Kim$^{10}$,
B.~Kimelman$^{8}$,
D.~Kincses$^{16}$,
T.~A.~Kinghorn$^{8}$,
I.~Kisel$^{17}$,
A.~Kiselev$^{6}$,
A.~Kisiel$^{60}$,
M.~Kocan$^{14}$,
L.~Kochenda$^{35}$,
L.~K.~Kosarzewski$^{14}$,
L.~Kramarik$^{14}$,
P.~Kravtsov$^{35}$,
K.~Krueger$^{4}$,
N.~Kulathunga~Mudiyanselage$^{20}$,
L.~Kumar$^{40}$,
R.~Kunnawalkam~Elayavalli$^{61}$,
J.~H.~Kwasizur$^{25}$,
R.~Lacey$^{51}$,
S.~Lan$^{11}$,
J.~M.~Landgraf$^{6}$,
J.~Lauret$^{6}$,
A.~Lebedev$^{6}$,
R.~Lednicky$^{28}$,
J.~H.~Lee$^{6}$,
Y.~H.~Leung$^{31}$,
C.~Li$^{47}$,
W.~Li$^{44}$,
W.~Li$^{49}$,
X.~Li$^{47}$,
Y.~Li$^{55}$,
Y.~Liang$^{29}$,
R.~Licenik$^{38}$,
T.~Lin$^{53}$,
Y.~Lin$^{11}$,
M.~A.~Lisa$^{39}$,
F.~Liu$^{11}$,
H.~Liu$^{25}$,
P.~ Liu$^{51}$,
P.~Liu$^{49}$,
T.~Liu$^{62}$,
X.~Liu$^{39}$,
Y.~Liu$^{53}$,
Z.~Liu$^{47}$,
T.~Ljubicic$^{6}$,
W.~J.~Llope$^{61}$,
R.~S.~Longacre$^{6}$,
N.~S.~ Lukow$^{52}$,
S.~Luo$^{12}$,
X.~Luo$^{11}$,
G.~L.~Ma$^{49}$,
L.~Ma$^{18}$,
R.~Ma$^{6}$,
Y.~G.~Ma$^{49}$,
N.~Magdy$^{12}$,
R.~Majka$^{62}$,
D.~Mallick$^{36}$,
S.~Margetis$^{29}$,
C.~Markert$^{54}$,
H.~S.~Matis$^{31}$,
J.~A.~Mazer$^{45}$,
N.~G.~Minaev$^{42}$,
S.~Mioduszewski$^{53}$,
B.~Mohanty$^{36}$,
M.~M.~Mondal$^{51}$,
I.~Mooney$^{61}$,
Z.~Moravcova$^{14}$,
D.~A.~Morozov$^{42}$,
M.~Nagy$^{16}$,
J.~D.~Nam$^{52}$,
Md.~Nasim$^{22}$,
K.~Nayak$^{11}$,
D.~Neff$^{9}$,
J.~M.~Nelson$^{7}$,
D.~B.~Nemes$^{62}$,
M.~Nie$^{48}$,
G.~Nigmatkulov$^{35}$,
T.~Niida$^{56}$,
L.~V.~Nogach$^{42}$,
T.~Nonaka$^{11}$,
G.~Odyniec$^{31}$,
A.~Ogawa$^{6}$,
S.~Oh$^{31}$,
V.~A.~Okorokov$^{35}$,
B.~S.~Page$^{6}$,
R.~Pak$^{6}$,
A.~Pandav$^{36}$,
Y.~Panebratsev$^{28}$,
B.~Pawlik$^{2}$,
D.~Pawlowska$^{60}$,
H.~Pei$^{11}$,
C.~Perkins$^{7}$,
L.~Pinsky$^{20}$,
R.~L.~Pint\'{e}r$^{16}$,
J.~Pluta$^{60}$,
J.~Porter$^{31}$,
M.~Posik$^{52}$,
N.~K.~Pruthi$^{40}$,
M.~Przybycien$^{2}$,
J.~Putschke$^{61}$,
H.~Qiu$^{26}$,
A.~Quintero$^{52}$,
S.~K.~Radhakrishnan$^{29}$,
S.~Ramachandran$^{30}$,
R.~L.~Ray$^{54}$,
R.~Reed$^{32}$,
H.~G.~Ritter$^{31}$,
J.~B.~Roberts$^{44}$,
O.~V.~Rogachevskiy$^{28}$,
J.~L.~Romero$^{8}$,
L.~Ruan$^{6}$,
J.~Rusnak$^{38}$,
N.~R.~Sahoo$^{48}$,
H.~Sako$^{56}$,
S.~Salur$^{45}$,
J.~Sandweiss$^{62}$,
S.~Sato$^{56}$,
W.~B.~Schmidke$^{6}$,
N.~Schmitz$^{33}$,
B.~R.~Schweid$^{51}$,
F.~Seck$^{15}$,
J.~Seger$^{13}$,
M.~Sergeeva$^{9}$,
R.~Seto$^{10}$,
P.~Seyboth$^{33}$,
N.~Shah$^{24}$,
E.~Shahaliev$^{28}$,
P.~V.~Shanmuganathan$^{6}$,
M.~Shao$^{47}$,
F.~Shen$^{48}$,
W.~Q.~Shen$^{49}$,
S.~S.~Shi$^{11}$,
Q.~Y.~Shou$^{49}$,
E.~P.~Sichtermann$^{31}$,
R.~Sikora$^{2}$,
M.~Simko$^{38}$,
J.~Singh$^{40}$,
S.~Singha$^{26}$,
N.~Smirnov$^{62}$,
W.~Solyst$^{25}$,
P.~Sorensen$^{6}$,
H.~M.~Spinka$^{4}$,
B.~Srivastava$^{43}$,
T.~D.~S.~Stanislaus$^{58}$,
M.~Stefaniak$^{60}$,
D.~J.~Stewart$^{62}$,
M.~Strikhanov$^{35}$,
B.~Stringfellow$^{43}$,
A.~A.~P.~Suaide$^{46}$,
M.~Sumbera$^{38}$,
B.~Summa$^{41}$,
X.~M.~Sun$^{11}$,
Y.~Sun$^{47}$,
Y.~Sun$^{21}$,
B.~Surrow$^{52}$,
D.~N.~Svirida$^{3}$,
P.~Szymanski$^{60}$,
A.~H.~Tang$^{6}$,
Z.~Tang$^{47}$,
A.~Taranenko$^{35}$,
T.~Tarnowsky$^{34}$,
J.~H.~Thomas$^{31}$,
A.~R.~Timmins$^{20}$,
D.~Tlusty$^{13}$,
M.~Tokarev$^{28}$,
C.~A.~Tomkiel$^{32}$,
S.~Trentalange$^{9}$,
R.~E.~Tribble$^{53}$,
P.~Tribedy$^{6}$,
S.~K.~Tripathy$^{16}$,
O.~D.~Tsai$^{9}$,
Z.~Tu$^{6}$,
T.~Ullrich$^{6}$,
D.~G.~Underwood$^{4}$,
I.~Upsal$^{48,6}$,
G.~Van~Buren$^{6}$,
J.~Vanek$^{38}$,
A.~N.~Vasiliev$^{42}$,
I.~Vassiliev$^{17}$,
F.~Videb{\ae}k$^{6}$,
S.~Vokal$^{28}$,
S.~A.~Voloshin$^{61}$,
F.~Wang$^{43}$,
G.~Wang$^{9}$,
J.~S.~Wang$^{21}$,
P.~Wang$^{47}$,
Y.~Wang$^{11}$,
Y.~Wang$^{55}$,
Z.~Wang$^{48}$,
J.~C.~Webb$^{6}$,
P.~C.~Weidenkaff$^{19}$,
L.~Wen$^{9}$,
G.~D.~Westfall$^{34}$,
H.~Wieman$^{31}$,
S.~W.~Wissink$^{25}$,
R.~Witt$^{57}$,
Y.~Wu$^{10}$,
Z.~G.~Xiao$^{55}$,
G.~Xie$^{31}$,
W.~Xie$^{43}$,
H.~Xu$^{21}$,
N.~Xu$^{31}$,
Q.~H.~Xu$^{48}$,
Y.~F.~Xu$^{49}$,
Y.~Xu$^{48}$,
Z.~Xu$^{6}$,
Z.~Xu$^{9}$,
C.~Yang$^{48}$,
Q.~Yang$^{48}$,
S.~Yang$^{6}$,
Y.~Yang$^{37}$,
Z.~Yang$^{11}$,
Z.~Ye$^{44}$,
Z.~Ye$^{12}$,
L.~Yi$^{48}$,
K.~Yip$^{6}$,
H.~Zbroszczyk$^{60}$,
W.~Zha$^{47}$,
D.~Zhang$^{11}$,
S.~Zhang$^{47}$,
S.~Zhang$^{49}$,
X.~P.~Zhang$^{55}$,
Y.~Zhang$^{47}$,
Y.~Zhang$^{11}$,
Z.~J.~Zhang$^{37}$,
Z.~Zhang$^{6}$,
J.~Zhao$^{43}$,
C.~Zhong$^{49}$,
C.~Zhou$^{49}$,
X.~Zhu$^{55}$,
Z.~Zhu$^{48}$,
M.~Zurek$^{31}$,
M.~Zyzak$^{17}$
}

\address{$^{1}$Abilene Christian University, Abilene, Texas   79699}
\address{$^{2}$AGH University of Science and Technology, FPACS, Cracow 30-059, Poland}
\address{$^{3}$Alikhanov Institute for Theoretical and Experimental Physics NRC "Kurchatov Institute", Moscow 117218, Russia}
\address{$^{4}$Argonne National Laboratory, Argonne, Illinois 60439}
\address{$^{5}$American University of Cairo, New Cairo 11835, New Cairo, Egypt}
\address{$^{6}$Brookhaven National Laboratory, Upton, New York 11973}
\address{$^{7}$University of California, Berkeley, California 94720}
\address{$^{8}$University of California, Davis, California 95616}
\address{$^{9}$University of California, Los Angeles, California 90095}
\address{$^{10}$University of California, Riverside, California 92521}
\address{$^{11}$Central China Normal University, Wuhan, Hubei 430079 }
\address{$^{12}$University of Illinois at Chicago, Chicago, Illinois 60607}
\address{$^{13}$Creighton University, Omaha, Nebraska 68178}
\address{$^{14}$Czech Technical University in Prague, FNSPE, Prague 115 19, Czech Republic}
\address{$^{15}$Technische Universit\"at Darmstadt, Darmstadt 64289, Germany}
\address{$^{16}$ELTE E\"otv\"os Lor\'and University, Budapest, Hungary H-1117}
\address{$^{17}$Frankfurt Institute for Advanced Studies FIAS, Frankfurt 60438, Germany}
\address{$^{18}$Fudan University, Shanghai, 200433 }
\address{$^{19}$University of Heidelberg, Heidelberg 69120, Germany }
\address{$^{20}$University of Houston, Houston, Texas 77204}
\address{$^{21}$Huzhou University, Huzhou, Zhejiang  313000}
\address{$^{22}$Indian Institute of Science Education and Research (IISER), Berhampur 760010 , India}
\address{$^{23}$Indian Institute of Science Education and Research (IISER) Tirupati, Tirupati 517507, India}
\address{$^{24}$Indian Institute Technology, Patna, Bihar 801106, India}
\address{$^{25}$Indiana University, Bloomington, Indiana 47408}
\address{$^{26}$Institute of Modern Physics, Chinese Academy of Sciences, Lanzhou, Gansu 730000 }
\address{$^{27}$University of Jammu, Jammu 180001, India}
\address{$^{28}$Joint Institute for Nuclear Research, Dubna 141 980, Russia}
\address{$^{29}$Kent State University, Kent, Ohio 44242}
\address{$^{30}$University of Kentucky, Lexington, Kentucky 40506-0055}
\address{$^{31}$Lawrence Berkeley National Laboratory, Berkeley, California 94720}
\address{$^{32}$Lehigh University, Bethlehem, Pennsylvania 18015}
\address{$^{33}$Max-Planck-Institut f\"ur Physik, Munich 80805, Germany}
\address{$^{34}$Michigan State University, East Lansing, Michigan 48824}
\address{$^{35}$National Research Nuclear University MEPhI, Moscow 115409, Russia}
\address{$^{36}$National Institute of Science Education and Research, HBNI, Jatni 752050, India}
\address{$^{37}$National Cheng Kung University, Tainan 70101 }
\address{$^{38}$Nuclear Physics Institute of the CAS, Rez 250 68, Czech Republic}
\address{$^{39}$Ohio State University, Columbus, Ohio 43210}
\address{$^{40}$Panjab University, Chandigarh 160014, India}
\address{$^{41}$Pennsylvania State University, University Park, Pennsylvania 16802}
\address{$^{42}$NRC "Kurchatov Institute", Institute of High Energy Physics, Protvino 142281, Russia}
\address{$^{43}$Purdue University, West Lafayette, Indiana 47907}
\address{$^{44}$Rice University, Houston, Texas 77251}
\address{$^{45}$Rutgers University, Piscataway, New Jersey 08854}
\address{$^{46}$Universidade de S\~ao Paulo, S\~ao Paulo, Brazil 05314-970}
\address{$^{47}$University of Science and Technology of China, Hefei, Anhui 230026}
\address{$^{48}$Shandong University, Qingdao, Shandong 266237}
\address{$^{49}$Shanghai Institute of Applied Physics, Chinese Academy of Sciences, Shanghai 201800}
\address{$^{50}$Southern Connecticut State University, New Haven, Connecticut 06515}
\address{$^{51}$State University of New York, Stony Brook, New York 11794}
\address{$^{52}$Temple University, Philadelphia, Pennsylvania 19122}
\address{$^{53}$Texas A\&M University, College Station, Texas 77843}
\address{$^{54}$University of Texas, Austin, Texas 78712}
\address{$^{55}$Tsinghua University, Beijing 100084}
\address{$^{56}$University of Tsukuba, Tsukuba, Ibaraki 305-8571, Japan}
\address{$^{57}$United States Naval Academy, Annapolis, Maryland 21402}
\address{$^{58}$Valparaiso University, Valparaiso, Indiana 46383}
\address{$^{59}$Variable Energy Cyclotron Centre, Kolkata 700064, India}
\address{$^{60}$Warsaw University of Technology, Warsaw 00-661, Poland}
\address{$^{61}$Wayne State University, Detroit, Michigan 48201}
\address{$^{62}$Yale University, New Haven, Connecticut 06520}
